Code Prompting Elicits Conditional Reasoning Abilities in Text+Code LLMs

Reasoning is a fundamental component of language understanding. Recent prompting techniques, such as chain of thought, have consistently improved LLMs' performance on various reasoning tasks. Nevertheless, there is still little understanding of what triggers reasoning abilities in LLMs in the inference stage. In this paper, we introduce code prompting, a chain of prompts that transforms a natural language problem into code and directly prompts the LLM using the generated code without resorting to external code execution. We hypothesize that code prompts can elicit certain reasoning capabilities of LLMs trained on text and code and utilize the proposed method to improve conditional reasoning, the ability to infer different conclusions depending on the fulfillment of certain conditions. We find that code prompting exhibits a high-performance boost for multiple LLMs (up to 22.52 percentage points on GPT 3.5, 7.75 on Mixtral, and 16.78 on Mistral) across multiple conditional reasoning datasets. We then conduct comprehensive experiments to understand how code prompts trigger reasoning abilities and which capabilities are elicited in the underlying models. Our analysis of GPT 3.5 reveals that the code formatting of the input problem is essential for performance improvement. Furthermore, code prompts improve sample efficiency of in-context learning and facilitate state tracking of variables or entities.

==> latex/new_tables/overall_results_dev.tex <==
\begin{table*}[t]
\renewcommand{\arraystretch}{0.85}
\begin{center}
\begin{tabular}{llccccccc}
\toprule
\textbf{Model} & \textbf{Prompt}                   & \textbf{CondQA} & \textbf{ShARC}     & \textbf{BGQA-1} & \textbf{BGQA-2} & \textbf{BGQA-3} \\
\midrule
\multirow{2}{*}{GPT 3.5} &Text           & $56.54\pm 0.08 $ & \textbf{63.91} $\pm$ \textbf{0.95} & $53.16 \pm 1.67$ & $33.71 \pm 10.37$  & $31.5 \pm 13.39$  \\
% &Text-3       & $56.35_{\pm 1.51}$ &  & $56.41 \pm 2.99$  & $51.79 \pm 2.42$ &  $42.68 \pm 0.58$  \\
&Code           & \textbf{57.64 $\pm$ 1.42} & 58.13 $\pm$ 1.62 &\textbf{68.60 $\pm$ 1.09} & \textbf{55.85 $\pm$ 4.06} & \textbf{47.57 $\pm$ 2.68}  \\

\multirow{2}{*}{Mixtral} &Text & \textbf{46.60} $\pm$ \textbf{0.99} & 53.55
 $\pm$ 1.58 & 58.31 $\pm$ 1.77  & 36.77 $\pm$ 0.09 & 32.06 $\pm$ 1.79  \\
&Code & 40.88 $\pm$ 1.84 & \textbf{58.03} $\pm$ \textbf{2.81} & 57.94 $\pm$ 5.52 & \textbf{45.32} $\pm$ \textbf{0.54} & \textbf{38.90} $\pm$ \textbf{7.33}  \\
\midrule

\multirow{2}{*}{Mistral} &Text & $28.84 \pm 0.02$ & 37.30 $\pm$ 1.69 & $47.61 \pm 0.92$ & $47.29 \pm 1.97$  & 46.56 $\pm$ 2.92 \\
&Code           & 28.26 $\pm$ 10.03 & \textbf{52.90} $\pm$ \textbf{1.08}  &\textbf{52.21} $\pm$ \textbf{0.95} & \textbf{54.27} $\pm$ \textbf{1.42} & 45.22 $\pm$ 10.75  \\

% \midrule
% \multirow{2}{*}{Phi-2} &Text & N.A. &   & $ 33.2 \pm 1.42 $  & N.A. &  N.A. \\
% &Code           & N.A. &  &\textbf{48.32} $\pm$ \textbf{1.65} & N.A. & N.A.  \\

\bottomrule
\end{tabular}
\end{center}
\caption{Comparison of text prompt and code prompts on the validation set of each dataset. Metric: F1 score. All results use one demonstration per class.}
\label{table:main_results_dev}
\end{table*}

==> latex/new_tables/overall_results_test.tex <==
\begin{table*}[t]
\renewcommand{\arraystretch}{0.85}
\begin{center}
\begin{tabular}{llccccccc}
\toprule
\textbf{Model} & \textbf{Prompt}                   & \textbf{CondQA} & \textbf{ShARC}     & \textbf{BGQA-1} & \textbf{BGQA-2} & \textbf{BGQA-3} \\
\midrule
\multirow{2}{*}{GPT 3.5} &Text  & 58.70 & \textbf{63.78} & 51.15  & 37.42  & 27.77  \\
                         &Code  & \textbf{60.60} & 59.54 & \textbf{58.67} & \textbf{55.56} & \textbf{50.29}  \\
\midrule

\multirow{2}{*}{Mixtral 8x7B} &Text & \textbf{48.17} & 60.29 & \textbf{56.38} & 39.64  & 30.15 \\
                         &Code & 44.73 & \textbf{62.77} & 53.33 & \textbf{47.39} &  \textbf{44.72} \\
\midrule

\multirow{2}{*}{Mistral 7B} &Text & \textbf{35.74}  & 37.70 & 47.40  & 48.78  & 47.86  \\
                         &Code & 32.28 & \textbf{54.48}  & \textbf{53.80} & \textbf{51.27}  & \textbf{48.79} \\

\bottomrule
\end{tabular}
\end{center}
\caption{Comparison of text prompt and code prompts on the test set of each dataset. Metric: F1 score. All results use one demonstration per class.}
\label{table:main_results_test}
\end{table*}

==> latex/tables/few_shot_reasoner_triggers.tex <==
\begin{table}[h]
\begin{center}
\scalebox{0.85}{
\begin{tabular}{lcccccc}
\toprule
\textbf{\# Ex.}                   & \textbf{CondQA}     & \textbf{Board-1} & \textbf{Board-2} & \textbf{Board-3} \\
\midrule
$\Delta$ 1 ex.           &  & $13.34$ & $11.66$ &   \\
$\Delta$ 2 ex.          &   &  &  &  \\
$\Delta$ 3 ex.           &   & 4.17 & 7.16 & 3  \\
\bottomrule
\end{tabular}
}
\end{center}
\caption{Comparison of the performance gap between code prompts and text prompts when using 1, 2, and 3 demonstrations per class.}
\label{table:few_shot_reasoner_trigger}
\end{table}

==> latex/tables/input_structure.tex <==
\begin{table*}[t]
\begin{center}
\begin{tabular}{lcccc}
\toprule
\textbf{Prompting Method} & \textbf{ConditionalQA} & \textbf{Board-1} & \textbf{Board-2} & \textbf{Board-3} \\
\midrule
Atomic Statements  & 55.94 & 57.80 & 47.80 & 35.6\\
Code $\rightarrow$ NL &  55.42 & 63.0 & 55.60 & 48.00 \\
\bottomrule
\end{tabular}
\end{center}
\caption{Analysis of the impact of the input format on the reasoning abilities of the LLM. \haritz{todo: remove this table and its references. this table merged with table 1}}
\label{table:input_structure}
\end{table*}

==> latex/tables/overall_results.tex <==
\begin{table*}[t]
\begin{center}
\begin{tabular}{lcccccc}
\toprule
\textbf{Prompt Method}                   & \textbf{CondQA}     & \textbf{BGQA-1} & \textbf{BGQA-2} & \textbf{BGQA-3} \\
\midrule
Text Prompt           & $56.32 \pm 1.06 $ & $62.80 \pm 0.28
$ & $55.00 \pm 0.56 $ & $47.59 \pm 0.00$  \\
Code Prompt           & \textbf{59.17 $\pm$ 0.74} & \textbf{69.40 $\pm$ 1.13} & \textbf{62.00 $\pm$ 1.70} & \textbf{55.30 $\pm$ 0.42}  \\
\midrule
Atomic Statements  & 55.94 & 57.80 & 47.80 & 35.60\\
Code $\rightarrow$ NL &  55.42 & 63.00 & 55.60 & 48.00 \\

\bottomrule
\end{tabular}
\end{center}
\caption{Comparison of text prompt and code prompts on the validation set of each dataset. Last two rows analyse the impact of the input format on text prompts.}
\label{table:main_results}
\end{table*}

==> latex/tables/qualitative_analysis.tex <==
\begin{table*}
    \centering
    \begin{tabular}{p{0.15\linewidth} | p{0.5\linewidth} | p{0.27\linewidth} }
    \toprule
         \textbf{Error Type} & \textbf{Example} & \textbf{Explanation} \\
         \midrule
         Commonsense &  We know the catfish has a harmonica, and according to Rule3 "\underline{if the catfish has something to sit on}, ... & The model believes a harmonica is something to sit on. \\
         Conditional Reasoning & \# We know the lion does not remove from the board one of the pieces of the dog, and according to Rule5 "if \underline{something becomes an enemy of the squid} but does not remove from the board one of the pieces of the dog, then it steals five points from the mosquito."
         
         \texttt{become\_enemy(lion, squid)==True}
        
         \texttt{not remove\_piece(lion, dog)==True}
        
         \texttt{steal\_points(lion,mosquito,5)=rule5(lion)}
        
         \texttt{steal\_points(lion, mosquito, 5)==True} & We do not know ~\texttt{become\_enemy(lion, squid) == True}, but if we assume this, we reach the question variable, so we get an answer to the question. \\
         \bottomrule
    \end{tabular}
    \caption{Examples of reasoning errors on correct instances by text and code prompts. Underline text is the cause of the error.}
    \label{table:qualitative_analysis}
\end{table*}


==> latex/tables/variable_tracking.tex <==
\begin{table*}[t]
    \centering
    \begin{tabular}{ccccc}
    \toprule
         &  \multicolumn{2}{c}{\textbf{Text Prompt}}&  \multicolumn{2}{c}{\textbf{Code Prompt}}\\
         \textbf{Dataset}&  \textbf{Correct Answers}&  \textbf{Wrong Answers}&  \textbf{Correct Answers}& \textbf{Wrong Answers}\\
         \midrule
         CondQA  & 71.08 & 60.79 & \textbf{4.39} & \textbf{11.39}\\
         BGQA-1 & 39.33 & 51.65  &  \textbf{8.84} & \textbf{22.12}\\
         BGQA-2 & 44.79 & 52.54 & \textbf{15.04} & \textbf{24.75} \\
         BGQA-3 & 54.01 & 52.13 & \textbf{14.21}  & \textbf{16.98}\\
    \bottomrule              

    \end{tabular}
    \caption{Comparison of the percentage of memory errors made by GPT 3.5. For each dataset, we calculate separately the memory errors for the instances where the model gives the correct and incorrect answers. Lower is better.}
    \label{tab:variable_tracking}
\end{table*}
